Learning Super-Resolution Ultrasound Localization Microscopy from Radio-Frequency Data

Ultrasound Localization Microscopy (ULM) enables imaging of vascular structures in the micrometer range by accumulating contrast agent particle locations over time. Precise and efficient target localization accuracy remains an active research topic in the ULM field to further push the boundaries of this promising medical imaging technology. Existing work incorporates Delay-And-Sum (DAS) beamforming into particle localization pipelines, which ultimately determines the ULM image resolution capability. In this paper we propose to feed unprocessed Radio-Frequency (RF) data into a super-resolution network while bypassing DAS beamforming and its limitations. To facilitate this, we demonstrate label projection and inverse point transformation between B-mode and RF coordinate space as required by our approach. We assess our method against state-of-the-art techniques based on a public dataset featuring in silico and in vivo data. Results from our RF-trained network suggest that excluding DAS beamforming offers a great potential to optimize on the ULM resolution performance.

==> figs/pala_sim_benchmark.tex <==
\begin{figure}[!ht]
  \centering
  \begin{minipage}[b]{0.242\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./img/pala_sim_results/gtru_ulm_img_15k_gam0.9.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./img/pala_sim_results/gtru_ulm_img_15k_gam0.9.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./img/pala_sim_results/gtru_ulm_img_15k_gam0.9.png}
    %\vspace{-.5cm}
    \subcaption{Ground Truth\label{fig:method1}}
    \vspace{+.1cm}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.242\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./img/pala_sim_results/pala_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./img/pala_sim_results/pala_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./img/pala_sim_results/pala_ulm_img_15k_gam0.9_128chs.png}
    %\vspace{-.5cm}
    \subcaption{RS~\{128\}~\cite{heiles2022pala}\label{fig:method2}}
    \vspace{+.1cm}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.242\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./img/pala_sim_results/unet_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./img/pala_sim_results/unet_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./img/pala_sim_results/unet_ulm_img_15k_gam0.9_128chs.png}
    %\vspace{-.5cm}
    \subcaption{U-Net~\{128\}~\cite{van2020super}\label{fig:method3}}
    \vspace{+.1cm}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.242\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./img/pala_sim_results/pace_ulm_img_15k_gam0.9_16chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./img/pala_sim_results/pace_ulm_img_15k_gam0.9_16chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./img/pala_sim_results/pace_ulm_img_15k_gam0.9_16chs.png}
    %\vspace{-.5cm}
    \subcaption{Ours~\{16\}\label{fig:method4}}
    \vspace{+.1cm}
  \end{minipage}
    \caption{Rendered ULM regions from Table~\ref{tab:benchmark} in (\subref{fig:method1}) to (\subref{fig:method4}) and a rat brain result in (\subref{fig:invivo}) without temporal tracking. Numbers in curly brackets indicate the transducer number.} %(full frames in Suppl. Material)
    \label{fig:render_ulm_crop}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

